Energy Efficient Hardware for On-Device CNN Inference via Transfer Learning

On-device CNN inference for real-time computer vision applications can result in computational demands that far exceed the energy budgets of mobile devices. This paper proposes FixyNN, a co-designed hardware accelerator platform which splits a CNN model into two parts: a set of layers that are fixed in the hardware platform as a front-end fixed-weight feature extractor, and the remaining layers which become a back-end classifier running on a conventional programmable CNN accelerator. The common front-end provides ubiquitous CNN features for all FixyNN models, while the back-end is programmable and specific to a given dataset. Image classification models for FixyNN are trained end-to-end via transfer learning, with front-end layers fixed for the shared feature extractor, and back-end layers fine-tuned for a specific task. Over a suite of six datasets, we trained models via transfer learning with an accuracy loss of <1%, resulting in a FixyNN hardware platform with nearly 2 times better energy efficiency than a conventional programmable CNN accelerator of the same silicon area (i.e. hardware cost).

==> methodology.tex <==
\section{Experimental Methodology}
\label{sec:methodology}

To evaluate FixyNN, we conduct experiments in both hardware modeling and transfer learning.
The hardware modeling experiments compare FixyNN against state-of-the-art hardware accelerator designs.
The transfer learning experiments evaluate generalization of a fixed feature extractor across a set of tasks.

% This work targets energy constrained CV tasks on mobile devices.
% We focus on image classification without loss of generality, since most fundamental CV operations such as object detection/localization and semantic segmentation tend to rely on image classification CNNs as a building block.
% % TODO give some examples here - YOLO/SSD for obj det and R-CNN for semantic segmentation???
% The experiments used for evaluation of FixyNN emphasize the MobileNet architecture for several reasons.
% As discussed previously, MobileNet is an efficient networkin terms of operations and 
% % TODO input patch size for mobilenet
% % TODO shove this in somewhere:
% MobileNet uses \textit{depth-wise separable layers}, which are composed of concatenated depth-wise $3 \times 3$ kernels and point-wise $1 \times 1 \times C$ kernels.
% FixyNN supports this layer type very efficiently by directly concatenating the depth-wise and point-wise kernels without any buffering, as the output dimensions of the depth-wise layer are the same as the input dimensions of the point-wise layer.


\subsection{Hardware Modeling}
\label{sec:methodology:hw}

FixyNN consists of two hardware components: the FFE, and a programmable CNN accelerator.
The FFE is generated using our ATOM tool (Section~\ref{sec:hw:atom}).
We use 8-bit precision for weights and activation data, and 32-bit maximum precision for accumulators.
For ASIC implementation experiments, we use Synopsys Design Compiler with TSMC 16nm FinFET process technology to characterize silicon area.
Timing analysis for throughput/latency is performed with Synposys PrimeTime.
All simulations use a clock frequency of 810 MHz.
Power characterization is performed using Synopsys PrimeTime PX with switching activity annotated from simulation trace data.

The programmable accelerator is based on published results for the NVIDIA Deep Learning Accelerator (NVDLA)~\cite{nvdla}.
NVDLA is a state-of-the-art open-source neural network accelerator, with Verilog RTL for hardware implementation and a TLM SystemC simulation model that can be used for software development, system integration, and testing.
NVDLA is configurable in terms of hardware resources.
Table~\ref{table:nvdla} summarizes the published performance of NVDLA in six nominal configurations.

% TODO - how did we model DRAM energy??

\begin{table}[ht]
\centering
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{c c c c c c}
\hline
Config. & \#MACs & Buffer (KB)	& 16nm Area (mm\textsuperscript{2})	& TOPS	& TOPS/W \\
\hline\hline
A	& 64		& 128		& 0.55		& 0.056		& 2.0 \\
B	& 128		& 256		& 0.84		& 0.156		& 3.8 \\
C	& 256		& 256		& 1.00		& 0.358		& 5.6 \\
D	& 512		& 256		& 1.40		& 0.728		& 6.8 \\
E	& 1024		& 256		& 1.80		& 1.166		& 6.3 \\
F	& 2048		& 512		& 3.30		& 2.095		& 5.4 \\
\hline
\end{tabular}}
\caption{Published NVDLA configurations, reproduced from~\cite{nvdla}.}
\label{table:nvdla}
\end{table}


% TODO I suspect that N is aliased parameter...
To explore the final FixyNN design space (Section~\ref{sec:results:hw}), we combine PPA models of an FFE containing the first \textit{N} layers of the network, along with the NVDLA programmable accelerator drawn from the published configurations.
ATOM is used to model the PPA of the fixed feature extractor.
% The FFE model is based on verified simulations of smaller networks.
% TODO - need to be careful with this - arguably sounds lazy??
Since the hardware performance of the FFE is heavily dependent on the sparsity of the network, we assume a cautious 50\% sparsity across the model for simplicity. 
Prior work has demonstrated that 50\% of weights can be pruned from MobileNet with minimal accuracy loss~\cite{prune_gupta17}.
The hardware modeling of NVDLA is from published data.
%programmable accelerator energy and latency utilizes throughput and efficiency measurements of NVDLA.
Because the latency of the FFE is much lower than that of the programmable NVDLA in the configurations we tested, we assume perfect clock gating in FixyNN to eliminate FFE power when idle.
Finally, we do not model FC layers as they are heavily memory bound and we would never be able to fix them anyway due to the huge number of parameters.

% TODO describe how we model DRAM cost and any other methodology details
% TODO - what's the paper we use to cite for the DRAM energy??????



\subsection{Transfer Learning}
\label{sec:methodology:ml}

% TODO
% Models can be trained and processed to optimize for both sparsity and Hamming weight.
% In this paper, we have not artificially optimized the models to emphasize weight sparsity or total Hamming weight, but leave this for future work.

The fixed feature extractor is constrained not only by silicon area considerations, but also by the achievable model accuracy.
The foundational work on transfer learning showed that as more layers are transfered, the accuracy becomes limited due to change in representational power and the later layers are more task specific than the early layers~\cite{yosinski_nips18}. 
In previous work, transfer learning is typically applied on big models such as AlexNet, which is prohibitively expensive from a hardware implementation point of view. 
Furthermore, it is arguably easier to perform transfer learning when the model capacity is very high as more parameters are available to fit the new dataset. 
In this paper, we perform a set of transfer learning experiments showing good performance with fixed weights on MobileNet, a much more constrained model.

Inspired by the \textit{visual decathlon challenge}~\cite{rebuffi_17} introduced to explore multiple-domain learning for image recognition, we choose seven different image recognition tasks to design our experiments: \textbf{ImageNet}~\cite{russakovsky2015imagenet}, \textbf{CIFAR-100}~\cite{krizhevsky2009learning}, \textbf{CIFAR-10}~\cite{krizhevsky2009learning}, \textbf{The Street View House Numbers (SVHN)}~\cite{netzer2011reading}, \textbf{Flowers102 (Flwr)}~\cite{nilsback2008automated}, \textbf{FGVC-Aircraft (Airc) Benchmark}~\cite{maji2013fine}, and \textbf{The German Traffic Sign Recognition (GTSR) Benchmark}~\cite{stallkamp2012man}. 
These datasets vary in number of images, resolution and granularity. For example, \textbf{ImageNet} and \textbf{CIFAR-100} are diverse datasets with a wide range of objects, while \textbf{Flwr} and \textbf{Airc} are fine-grained recognition tasks for specific vision domains of flowers and aircrafts respectively.

For the first set of experiments, we use MobileNet-$0.25$, an efficient model with only $41$ million MACs and $0.47$ million parameters. 
The model is first trained on \textbf{ImageNet} to an accuracy of $49.8\%$ (state-of-the-art for this small MobileNet model) and then transfered to the other six vision tasks. 
The baseline results are obtained by performing full-fledged fine-tuning, where all the parameters of the model are updated during fine-tuning on the new dataset. 
This is used as the baseline case for a model running on a programmable DLA. 
Six different FixyNN topologies are explored in these experiments, with different number of layers being fixed. 
In some topologies, all batch normalization layer scaling and bias parameters in the model are retrained on the new dataset. 
We call this configuration Adaptive Batch-Normalization (BN).

Stochastic gradient descent with an initial learning rate of $0.01$ and momentum of $0.9$ is used to perform fine-tuning (except for GTSR dataset, where an initial learning rate of $0.001$ is used for better convergence). 
The learning rate is decayed $10 \times$ every $100$ epochs (200 epochs for GTSR). 
A batch size of $128$ is used. The seven datasets come with different resolutions. 
For the purpose of standardization, all images are resized to $224\times224$ using bilinear interpolation. 
Data augmentation preproccessing is applied to all datasets. Random color distortion, flipping and cropping are applied. 
Horizontal left-right flipping is turned off for datasets \textbf{SVHN} and \textbf{GTSR}, cropping ratio is also increased as these two datasets are street number and traffic sign photos. 
MobileNet-$0.25$ is a limited capacity model so little regularization is required. 
Weight decay of $4 \times 10^{-5}$ is used in fine-tuning ($4 \times 10^{-4}$ for GTSR).

To demonstrate generalization of this approach, a second set of experiments are carried out using MobileNet-$1.0$. 
MobileNet-$1.0$ has $569$ million MACs and $4.24$ million parameters, which is about $10\times$ bigger than MobileNet-$0.25$. 
It is trained on \textbf{ImageNet} to an accuracy of $70.9\%$. 
We only transfer this model to \textbf{CIFAR100} to showcase the similar trend of transfer learning performance for a bigger model. 
%We shall see that the required area becomes expensive with a bigger CNN model.



